Is the Regge Calculus a consistent approximation to General Relativity?

We will ask the question of whether or not the Regge calculus (and two related simplicial formulations) is a consistent approximation to General Relativity. Our criteria will be based on the behaviour of residual errors in the discrete equations when evaluated on solutions of the Einstein equations. We will show that for generic simplicial lattices the residual errors can not be used to distinguish metrics which are solutions of Einstein's equations from those that are not. We will conclude that either the Regge calculus is an inconsistent approximation to General Relativity or that it is incorrect to use residual errors in the discrete equations as a criteria to judge the discrete equations.

==> 10ptsgl.tex <==
%
\catcode`@=11%
%
\def\defineten{%
   \font\tentext=cmr10 scaled 1000%
   \font\tenscript=cmr7 scaled 1000%
   \font\tenscriptscript=cmr5 scaled 1000%
   \font\tenmathtext=cmmi10 scaled 1000%
   \font\tenmathscript=cmmi7 scaled 1000%
   \font\tenmathscriptscript=cmmi5 scaled 1000%
   \font\tensymboltext=cmsy10 scaled 1000%
   \font\tensymbolscript=cmsy7 scaled 1000%
   \font\tensymbolscriptscript=cmsy5 scaled 1000%
   \font\tenmathex=cmex10 scaled 1000%
   \font\tenboldtext=cmbx10 scaled 1000%
   \font\tenboldscript=cmbx7 scaled 1000%
   \font\tenboldscriptscript=cmbx5 scaled 1000%
   \font\tenslant=cmsl10 scaled 1000%
   \font\tenitalic=cmti10 scaled 1000%
   \font\tentypewriter=cmtt10 scaled 1000%
% Set skew and hyphenation characters
   \skewchar\tenmathtext='177%
   \skewchar\tenmathscript='177%
   \skewchar\tenmathscriptscript='177%
   \skewchar\tensymboltext='60%
   \skewchar\tensymbolscript='60%
   \skewchar\tensymbolscriptscript='60%
   \hyphenchar\tentypewriter=-1%
}% \global\let\defineten=\relax}%
%
\def\tenpoint{%
   \defineten%
   \textfont0=\tentext \scriptfont0=\tenscript%
      \scriptscriptfont0=\tenscriptscript%
   \def\rm{\fam0 \tentext}%%
   \textfont1=\tenmathtext \scriptfont1=\tenmathscript%
      \scriptscriptfont1=\tenmathscriptscript%
   \textfont2=\tensymboltext \scriptfont2=\tensymbolscript%
      \scriptscriptfont2=\tensymbolscriptscript%
   \textfont3=\tenmathex \scriptfont3=\tenmathex%
      \scriptscriptfont3=\tenmathex%
   \textfont\bffam=\tenboldtext \scriptfont\bffam=\tenboldscript%
      \scriptscriptfont\bffam=\tenboldscriptscript%
   \def\bf{\fam\bffam\tenboldtext}%
   \textfont\itfam=\tenitalic \def\it{\fam\itfam\tenitalic}%
   \textfont\slfam=\tenslant \def\sl{\fam\slfam\tenslant}%
   \textfont\ttfam=\tentypewriter \def\tt{\fam\ttfam\tentypewriter}%
%Set up \mit, \oldstyle, \cal
   \def\mit{\fam1 }\def\oldstyle{\fam1 \tenmathtextfont}%
   \def\cal{\fam2 }%
%Set up big etc.
\def\big##1{{\hbox{$\left##1\vbox to 8.5pt{}\right.\n@space$}}}%
\def\Big##1{{\hbox{$\left##1\vbox to 11.5pt{}\right.\n@space$}}}%
\def\bigg##1{{\hbox{$\left##1\vbox to 14.5pt{}\right.\n@space$}}}%
\def\Bigg##1{{\hbox{$\left##1\vbox to 17.5pt{}\right.\n@space$}}}%
%
%Now define a strut box for tenpt
   \setbox\strutbox=\hbox{\vrule height 8.5pt depth 3.5pt width0pt}%
   \normalbaselineskip=12pt%
   \normalbaselines\rm%
}
%
\catcode`@=12% Back to normal

